A mean-field game price model with noise

In this paper, we propose a mean-field game model for the price formation of a commodity whose production is subjected to random fluctuations. The model generalizes existing deterministic price formation models. Agents seek to minimize their average cost by choosing their trading rates with a price that is characterized by a balance between supply and demand. The supply and the price processes are assumed to follow stochastic differential equations. Here, we show that, for linear dynamics and quadratic costs, the optimal trading rates are determined in feedback form. Hence, the price arises as the solution to a stochastic differential equation, whose coefficients depend on the solution of a system of ordinary differential equations.

==> mfgtemp.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Rita A. Ferreira at 2019-04-01 14:06:57 +0300 


%% Saved with string encoding Unicode (UTF-8) 


@comment{jabref-meta: databaseType:bibtex;}
@preamble{"\def\cprime{$'$} "}


@article{Ahuja_2016,
   title={Wellposedness of Mean Field Games with Common Noise under a Weak Monotonicity Condition},
   volume={54},
   ISSN={1095-7138},
   url={http://dx.doi.org/10.1137/140974730},
   DOI={10.1137/140974730},
   number={1},
   journal={SIAM Journal on Control and Optimization},
   publisher={Society for Industrial & Applied Mathematics (SIAM)},
   author={Ahuja, Saran},
   year={2016},
   month={Jan},
   pages={30–48}
}

@article{bensoussan2014linearquadratic,
    title={Linear-Quadratic Mean Field Games},
    author={Alain Bensoussan and Joseph Sung and Phillip Yam and Siu Pang Yung},
    year={2014},
    eprint={1404.5741},
    archivePrefix={arXiv},
    primaryClass={math.OC}
}

@article{carmona2016,
author = "Carmona, René and Delarue, François and Lacker, Daniel",
doi = "10.1214/15-AOP1060",
fjournal = "The Annals of Probability",
journal = "Ann. Probab.",
month = "11",
number = "6",
pages = "3740--3803",
publisher = "The Institute of Mathematical Statistics",
title = "Mean field games with common noise",
url = "https://doi.org/10.1214/15-AOP1060",
volume = "44",
year = "2016"
}

@misc{carmona2013mean,
    title={Mean Field Games and Systemic Risk},
    author={Rene Carmona and Jean-Pierre Fouque and Li-Hsien Sun},
    year={2013},
    eprint={1308.2172},
    archivePrefix={arXiv},
    primaryClass={q-fin.PR}
}



@misc{coghi2019stochastic,
    title={Stochastic nonlinear Fokker-Planck equations},
    author={Michele Coghi and Benjamin Gess},
    year={2019},
    eprint={1904.07894},
    archivePrefix={arXiv},
    primaryClass={math.PR}
}

@misc{kolokoltsov2015mean,
    title={On the mean field games with common noise and the McKean-Vlasov SPDEs},
    author={Vassili Kolokoltsov and Marianna Troeva},
    year={2015},
    eprint={1506.04594},
    archivePrefix={arXiv},
    primaryClass={math.PR}
}



